Diverse Complexity Measures for Dataset Curation in Self-driving

Modern self-driving autonomy systems heavily rely on deep learning. As a consequence, their performance is influenced significantly by the quality and richness of the training data. Data collecting platforms can generate many hours of raw data in a daily basis, however, it is not feasible to label everything. It is thus of key importance to have a mechanism to identify "what to label". Active learning approaches identify examples to label, but their interestingness is tied to a fixed model performing a particular task. These assumptions are not valid in self-driving, where we have to solve a diverse set of tasks (i.e., perception, and motion forecasting) and our models evolve over time frequently. In this paper we introduce a novel approach and propose a new data selection method that exploits a diverse set of criteria that quantize interestingness of traffic scenes. Our experiments on a wide range of tasks and models show that the proposed curation pipeline is able to select datasets that lead to better generalization and higher performance.

==> sections/tables/plan.tex <==

\begin{table*}[t]
	\centering
		\scriptsize
		\begin{threeparttable}
			\begin{tabularx}{\textwidth}{
				>{\centering\arraybackslash}c |  %
				>{\centering\arraybackslash}X |
				>{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X}
			\toprule
            Model 	              &  Dataset size   &  Human L2@3sec  & Collision@3sec (\%) & Jerk\\
			\midrule
			\multirow{2}{*}{NMP\cite{zeng2019end}} 				  &1k&-&-&-\\
                                                       &3k&-&-&-\\
            \midrule
            \multirow{2}{*}{P3\cite{sadat2020perceive}} 					  &1k&-&-&-\\
                                                        &3k&-&-&-\\
			\midrule
			\multirow{2}{*}{PLT\cite{sadat2019jointly}} 					  &1k&-&-&-\\
														&3k&-&-&-\\
            
			\bottomrule
			\end{tabularx}
		\end{threeparttable}
    \caption{Planning task}
    \label{tbl:planning}
\end{table*}
